Unifying Tree Search Algorithm and Reward Design for LLM Reasoning: A Survey

Deliberative tree search is a cornerstone of modern Large Language Model (LLM) research, driving the pivot from brute-force scaling toward algorithmic efficiency. This single paradigm unifies two critical frontiers: \textbf{Test-Time Scaling (TTS)}, which deploys on-demand computation to solve hard problems, and \textbf{Self-Improvement}, which uses search-generated data to durably enhance model parameters. However, this burgeoning field is fragmented and lacks a common formalism, particularly concerning the ambiguous role of the reward signal -- is it a transient heuristic or a durable learning target? This paper resolves this ambiguity by introducing a unified framework that deconstructs search algorithms into three core components: the \emph{Search Mechanism}, \emph{Reward Formulation}, and \emph{Transition Function}. We establish a formal distinction between transient \textbf{Search Guidance} for TTS and durable \textbf{Parametric Reward Modeling} for Self-Improvement. Building on this formalism, we introduce a component-centric taxonomy, synthesize the state-of-the-art, and chart a research roadmap toward more systematic progress in creating autonomous, self-improving agents.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tree_taxonomy.tex <==
\begin{figure*}[!b]
    % \vspace{-2mm}
    \centering
    \resizebox{0.96\textwidth}{!}{
    \begin{forest}
        forked edges,
        for tree={
            grow=east,
            reversed=true,
            anchor=base west,
            parent anchor=east,
            child anchor=west,
            base=left,
            font=\large,
            rectangle,
            draw=hidden-black,
            rounded corners,
            align=left,
            minimum width=4em,
            edge+={darkgray, line width=1pt},
            s sep=3pt,
            inner xsep=2pt,
            inner ysep=4pt,
            line width=1.1pt,
            ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
        },
        where level=1{text width=9.5em,font=\normalsize,}{},
        where level=2{text width=11.5em,font=\normalsize,}{},
        where level=3{text width=12em,font=\normalsize,}{},
        % Level 4 styling is now handled by leaf3
        [Taxonomy, ver
            [MCTS for \\ Direct Test-Time \\ Enhancement
                [General Reasoning \\ \& Problem Solving
                    [{ 
                        Discriminator-based Tree Search~\citep{chen2024tree}, 
                        Interpretable Contrastive MCTS~\citep{gao2024interpretable}, \\
                        RoT~\citep{hui2024rot}, 
                        LiteSearch~\citep{wang2024litesearch}, 
                        MindStar~\citep{kang2024mindstar}, \\
                        MARCO-O1~\citep{zhao2024marco}, 
                        Everything of Thoughts~\citep{ding2023everything}, 
                        CoAT~\citep{pan2025coat} 
                    }, leaf3]
                ]
                [Mathematical Reasoning
                    [{ 
                        MCTS Self-Refine~\citep{zhang2024accessing}, 
                        Energy Function MCTS~\citep{xu2023no}, 
                        OVM~\citep{yu2023ovm},  \\
                        LLaMA-Berry~\citep{zhang2025llama}, 
                        Automated Process Supervision~\citep{luo2024improve}, \\
                        Constrained MCTS~\citep{lin2025leveraging},  
                        Markov Chain of Thought~\citep{yang2024markov} \\
                    }, leaf3]
                ]
                [Code Generation \\ \& Software Engineering
                    [{ 
                        RTL Code Gen MCTS~\citep{delorenzo2024make}, 
                        RethinkMCTS~\citep{li2024rethinkmcts},  \\
                        Verified Multi-step Synthesis~\citep{brandfonbrener2024verified},
                        VerMCTS~\citep{brandfonbrener2024vermcts},    \\
                        Code World Models MCTS~\citep{dainese2024generating}, 
                        Planning in NL~\citep{wang2024planning},  \\
                        O1-Coder~\citep{zhang2024o1}, 
                        SRA-MCTS~\citep{xu2024sra}, 
                        SWE-Search~\citep{antoniades2024swe}, \\
                        SWE-Debate~\citep{li2025swe},  
                        MCTS-Judge~\citep{wang2025mcts}, \\
                        APRMCTS~\citep{hu2025aprmcts}, 
                        MCTS-Refined CoT~\citep{wang2025mcts}
                    }, leaf3]
                ]
                [LLM Agents \\ \& Interactive Environments
                    [{ 
                        LATS~\citep{zhou2023language}, 
                        SeLa~\citep{chi2024sela}, 
                        BIDA~\citep{yu2025bida}, \\
                        WebPilot~\citep{zhang2025webpilot}, 
                        Prompt-based MCTS~\citep{yu2023prompt}, 
                        MASTER~\citep{gan2025master},  \\
                        SE-Agent~\citep{lin2025se}, 
                        WebSynthesis~\citep{gao2025websynthesis},  \\
                        AgentSwift~\citep{li2025agentswift}, 
                        HALO~\citep{hou2025halo} 
                    }, leaf3]
                ]
                [Knowledge-Intensive \\ \& RAG Tasks
                    [{ 
                        KNOT-MCTS~\citep{wu2023knot}, 
                        Search-in-the-Chain~\citep{xu2024search}, \\
                        Contrastive RAG~\citep{gu2025toward}, 
                        RARE~\citep{tran2024rare}, 
                        CoRaG~\citep{wang2024corag}, \\
                        RITEK~\citep{huang2024ritek}, 
                        AirRAG~\citep{feng2025airrag}, 
                        KBQA-O1~\citep{luo2025kbqa}, \\
                        MCTS-KBQA~\citep{xiong2025mcts}, 
                        Hierarchical RAG~\citep{dou2025enhancing}, \\ 
                        Explainable MCTS~\citep{kowalski2025towards}, 
                        KCTS~\citep{choi2023kcts}, \\
                        RAG-Star~\citep{jiang2024rag},
                        FREESON~\citep{kim2025freeson} 
                    }, leaf3]
                ]
                [Multimodal Reasoning
                    [{ 
                        Mulberry~\citep{yao2024mulberry}, 
                        Progressive Multimodal Reasoning~\citep{dong2024progressive}, \\
                        MCTS-Automated Structured Thinking~\citep{wu2025boosting}, 
                        Dyfo~\citep{li2025dyfo} 
                    }, leaf3]
                ]
            ]
            [MCTS for \\ Self-Improvement \\ via Data Generation
                [ Self-Improvement \\ Foundational Frameworks
                    [{rStar-Math~\citep{guan2025rstar}, 
                    Alphazero-like tree-search~\citep{feng2023alphazero}, \\
                    Curriculum Preference Learning~\citep{wang2024towards}, 
                    Agent Q~\citep{putta2024agent},\\
                    Iterative Preference Learning~\citep{xie2024monte}, 
                    Imagination, Searching, and Criticizing~\citep{tian2024toward}, \\
                    Mutual Reasoning~\citep{qi2024mutual}, 
                    AlphaMath Almost Zero~\citep{chen2024alphamath}, 
                    CPL~\citep{wang2024cpl}, \\
                    Step-level Value Preference Optimization~\citep{chen2024step}, TreeRPO~\citep{yang2025treerpo}, \\
                    Data Influence-Oriented Tree Search~\citep{shi2025efficient}, 
                    MCTS-Refined CoT~\citep{wang2025mcts},  \\
                    ASTRO~\citep{kim2025astro}, 
                    % Agent-R~\citep{yuan2025agent},
                    }, leaf ]
                ]
                [General Capabilities \\ \& Alignment
                    [{PPL-MCTS~\citep{chaffin2021ppl}, Value-Guided MCTS~\citep{liu2023don}, ARGS~\citep{khanov2024args},  \\ Reflective Tree Search~\citep{yu2024improving}, PromptAgent~\citep{wang2023promptagent}, STAIR~\citep{zhang2025stair}, \\ 
                    Dynamic Rewarding~\citep{singla2024dynamic},  
                    Evolutionary Space Search~\citep{li2024optimizing},  \\
                    APRMCTS~\citep{hu2025aprmcts}}, leaf ]
                ]
                [Scientific \\ \& Specialized Domains
                    [{Self-Play Approach~\citep{guo2024can}, Named Entity Matching~\citep{volkova2024novel},  \\Synthetic Data Generation~\citep{locowic2024synthetic},  
                    Monte Carlo Thought Search~\citep{sprueill2023monte},  \\
                    STRATEGIST~\citep{light2024strategist}, Fast and Slow Thinking~\citep{cheng2025think},  Peptune~\citep{tang2025peptune}, \\
                    Multi-Agent Sampling~\citep{ye2024multi}, 
                    Step-level~\citep{ma2025step}, \\
                    Process Reward-guided Tree Search~\citep{park2024ensembling}, {Think\&Cite}~\citep{li2024think},  
                    SAPIENT~\citep{du2024sapient}, \\
                    Automatic Heuristic Design~\citep{zheng2025monte}, 
                    Trans-Zero~\citep{zou2025trans}, \\
                    Prompt-Based MCTS~\citep{duan2025prompt}, {MedS$^3$}~\citep{jiang2025meds},  
                    MCTSr-Zero~\citep{lu2025mctsr}, \\
                    K-MSE~\citep{zhuang-etal-2025-boosting} 
                    Stepwise Domain Knowledge-Driven Reasoning~\citep{liu2025towards} \\
                    IRIS~\citep{garikaparthi2025iris}, 
                    ChemAgent~\citep{wu2025chemagent}}, 
                    leaf ]
                ]
                [Multimodal Applications
                    [{MCTS-guided Sample Selection~\citep{wang2025sota}, MMC~\citep{liu2025mmc}, MM-PRM~\citep{du2025mm}}, leaf ]
                ]
            ]
            [Advanced Topics and \\ Hybrid Approaches
                [Multi-Agent and \\ Collaborative Search
                    [{Reflective Tree Search~\cite{yu2024improving}, 
                    Multi-agent sampling~\cite{ye2024multi}, \\
                    Process reward-guided tree search~\cite{park2024ensembling}, Webpilot~\cite{zhang2025webpilot}, 
                    MASTER~\cite{gan2025master}, \\
                    Data Influence-Oriented Tree Search~\cite{shi2025efficient}, 
                    Multi-LLM collaborative search~\cite{yang2025multi}, \\
                    KompeteAI~\cite{kulibaba2025kompeteai}, 
                    SWE-Debate~\cite{li2025swe}, \\
                    AniMaker~\cite{shi2025animaker}, 
                    HALO~\cite{hou2025halo}}, leaf4]
                ]
                [Reward Model Design \\ and Optimization
                    [{rStar-Math~\cite{guan2025rstar}, 
                    AlphaZero-like tree-search~\cite{feng2023alphazero}, \\
                    Iterative preference learning~\cite{xie2024monte}, 
                    Step-level q-value models~\cite{zhai2025enhancing}, \\
                    Curriculum Preference Learning~\cite{wang2024towards},
                    Interpretable contrastive MCTS~\cite{gao2024interpretable}, \\
                    Energy function guided MCTS~\cite{xu2023no}, 
                    AlphaMath Almost Zero~\cite{chen2024alphamath}, \\
                    CPL~\cite{wang2024cpl}, 
                    OVM~\cite{yu2023ovm}, 
                    Value-Guided MCTS~\cite{liu2023don},\\
                    Step-Level reward model~\cite{ma2023let}, 
                    Step-level value preference optimization~\cite{chen2024step}, \\
                    Automated process supervision~\cite{luo2024improve}, 
                    MCTS-boosted mathematical reasoning~\cite{ma2025step}, \\
                    {Think\&Cite}~\cite{li2024think}, 
                    STAIR~\cite{zhang2025stair}, 
                    MT-RewardTree~\cite{feng2025mt}, \\
                    Hierarchical Multi-Step Reward Models~\cite{wang2025towards}, 
                    ProMed~\cite{ding2025promed}, \\
                    TreeRPO~\cite{yang2025treerpo}, 
                    Unifying RL and Search-Based TTS~\cite{jin2025your},\\
                    Re-ranking Reasoning Context with Tree Search~\cite{yang2025re}
                    }, leaf4]
                ]
                [Search Efficiency \\ and Dynamics
                    [{Tree search for agents~\cite{koh2024tree}, 
                    Discriminator-dependent tree search~\cite{chen2024tree}, \\
                    Information Directed Tree Search~\cite{chandak2024information}, 
                    RoT~\cite{hui2024rot}, 
                    LiteSearch~\cite{wang2024litesearch},  \\
                    BoostStep~\cite{zhang2025booststep}, 
                    Everything of Thoughts~\cite{ding2023everything}, \\
                    Dual process of fast and slow thinking~\cite{cheng2025think}, 
                    T-SCEND~\cite{zhang2025t}, \\
                    BFS-Prover~\cite{xin2025bfs}, 
                    MCTS-Judge~\cite{wang2025mcts}, \\
                    Adaptive branching tree search~\cite{inoue2025wider}, 
                    Retro-Search~\cite{lu2025retro}, \\
                    Bilevel MCTS~\cite{asai2025bilevel}, 
                    Test-Time Depth Adaptation~\cite{li2025skip}, \\
                    Abstraction dropping methods~\cite{schmocker2025time}, 
                    SIGMA~\cite{ren2025sigma}, 
                    AgentSwift~\cite{li2025agentswift}, \\
                    FREESON~\cite{kim2025freeson}, 
                    Structural Entropy Guided Agent~\cite{wei2025structural}
                    }, leaf4]
                ]   
            ]
        ]
    \end{forest}
    }
    \caption{A comprehensive taxonomy of MCTS.}
    \label{fig:MCTS-taxonomy}
\end{figure*}

